How to Find Your Friendly Neighborhood: Graph Attention Design with Self-Supervision

Attention mechanism in graph neural networks is designed to assign larger weights to important neighbor nodes for better representation. However, what graph attention learns is not understood well, particularly when graphs are noisy. In this paper, we propose a self-supervised graph attention network (SuperGAT), an improved graph attention model for noisy graphs. Specifically, we exploit two attention forms compatible with a self-supervised task to predict edges, whose presence and absence contain the inherent information about the importance of the relationships between nodes. By encoding edges, SuperGAT learns more expressive attention in distinguishing mislinked neighbors. We find two graph characteristics influence the effectiveness of attention forms and self-supervision: homophily and average degree. Thus, our recipe provides guidance on which attention design to use when those two graph characteristics are known. Our experiment on 17 real-world datasets demonstrates that our recipe generalizes across 15 datasets of them, and our models designed by recipe show improved performance over baselines.

==> ICLR2021 (SuperGAT) (Arxiv)/files/big_table.tex <==

% Large result table padding guide
% \setlength{\tabcolsep}{3.1pt} % Default value: 6pt
% \def\arraystretch{1.6} % default: 1.0
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.1pt} % Default value: 6pt
\def\arraystretch{1.4} % default: 1.0
\caption{Summary of classification accuracies of GCN, GraphSAGE, GAT, \SuperGATSD, and \SuperGATMXb for real-world datasets (30 runs for ogbn-arxiv and Flickr, and 100 runs for others).}
\vspace{-0.2cm}
\label{tab:real-world-many}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllll}
\hline
Model &
  ogbn-arxiv &
  CS &
  Physics &
  Cora-ML &
  Cora-Full &
  DBLP &
  Cham. &
  Four-Univ &
  Wiki-CS &
  Photo &
  Comp. &
  Flickr &
  Croco. \\ \hline
GCN &
  $33.3_{\pm 1.2}$ &
  $91.5_{\pm 0.2}$ &
  $92.5_{\pm 0.2}$ &
  $85.0_{\pm 0.4}$ &
  $59.5_{\pm 0.2}$ &
  $77.8_{\pm 0.5}$ &
  $33.1_{\pm 0.9}$ &
  $74.8_{\pm 0.6}$ &
  $74.0_{\pm 1.0}$ &
  $91.6_{\pm 0.6}$ &
  $84.5_{\pm 1.4}$ &
  $51.2_{\pm 0.4}$ &
  $32.6_{\pm 0.4}$ \\
GraphSAGE &
  $54.6_{\pm 0.3}$ &
  $90.0_{\pm 0.1}$ &
  $92.2_{\pm 0.1}$ &
  $83.7_{\pm 0.4}$ &
  $59.2_{\pm 0.2}$ &
  $78.7_{\pm 0.6}$ &
  $41.0_{\pm 0.9}$ &
  $74.4_{\pm 0.6}$ &
  $77.5_{\pm 0.5 }$ &
  $90.4_{\pm 1.1}$ &
  $83.0_{\pm 1.4 }$ &
  $50.7_{\pm 0.2}$ &
  $53.0_{\pm 1.0}$ \\ \hline \hline
GAT &
  $54.1_{\pm 0.5}$ &
  $89.5_{\pm 0.2}$ &
  $91.2_{\pm 0.6}$ &
  $83.2_{\pm 0.6}$ &
  $58.7_{\pm 0.3}$ &
  $78.2_{\pm 1.5}$ &
  $40.8_{\pm 0.7}$ &
  $74.2_{\pm 0.7}$ &
  $77.6_{\pm 0.6}$ &
  \cellwg$\mathbf{91.8}_{\pm 0.6}$ &
  \cellwg$\mathbf{85.7}_{\pm 0.9}$ &
  \cellwg$\mathbf{50.9}_{\pm 0.2}$ &
  \cellwg$\mathbf{53.3}_{\pm 1.0}$ \\ \hline
\SuperGATSD &
  $54.5_{\pm 0.3}^{**}$ &
  $88.8_{\pm 0.4}^{\downarrow}$ &
  $91.6_{\pm 0.5}^{**}$ &
  $84.5_{\pm 0.4}^{**}$ &
  $55.8_{\pm 0.6}^{\downarrow}$ &
  $79.4_{\pm 0.8}^{**}$ &
  $41.6_{\pm 0.7}^{**}$ &
  \cellwb$\mathbf{76.2}_{\pm 0.8}^{**}$ &
  \cellwp$\mathbf{77.9}_{\pm 0.7}$ &
  \cellwg$86.8_{\pm 2.5}^{\downarrow}$ &
  \cellwg$82.2_{\pm 0.9}^{\downarrow}$ &
  \cellwg$45.1_{\pm 1.2}^{\downarrow}$ &
  \cellwg$\mathbf{53.3}_{\pm 0.9}$ \\
\SuperGATMX &
  \cellwr$\mathbf{55.1}_{\pm 0.2}^{**}$ &
  \cellwr$\mathbf{90.2}_{\pm 0.2}^{**}$ &
  \cellwr$\mathbf{91.9}_{\pm 0.5}^{**}$ &
  \cellwr$\mathbf{84.7}_{\pm 0.4}^{**}$ &
  \cellwr$\mathbf{59.6}_{\pm 0.2}^{**}$ &
  \cellwr$\mathbf{80.7}_{\pm 0.7}^{**}$ &
  \cellwr$\mathbf{42.0}_{\pm 0.8}^{**}$ &
  $75.3_{\pm 0.6}^{**}$ &
  \cellwp$\mathbf{77.9}_{\pm 0.5}^{*}$ &
  \cellwg$\mathbf{91.8}_{\pm 0.9}$ &
  \cellwg$\mathbf{85.7}_{\pm 1.1}$ &
  \cellwg$50.8_{\pm 0.2}^{\downarrow}$ &
  \cellwg$\mathbf{53.3}_{\pm 0.9}$ \\ \hline
\end{tabular}%
}
\vspace{-0.2cm}
\end{table}

==> ICLR2021 (SuperGAT) (Arxiv)/files/conclusion.tex <==
We proposed novel graph neural architecture designs to self-supervise graph attention following the input graph's characteristics. We first assessed what graph attention is learning and analyzed the effect of edge self-supervision to link prediction and node classification performance. This analysis showed two widely used attention mechanisms (original GAT and dot-product) have difficulty encoding label-agreement and edge presence simultaneously. To address this problem, we suggested several graph attention forms that balance these two factors and argued that graph attention should be designed depending on the input graph's average degree and homophily. Our experiments demonstrated that our graph attention recipe generalizes across various real-world datasets such that the models designed according to the recipe outperform other baseline models.

==> ICLR2021 (SuperGAT) (Arxiv)/files/experiments.tex <==
Our primary research objective is to design graph attentions that are effective with edge self-supervision. To do this, we pose four specific research questions. We first analyze what basic graph attentions (GO and DP) learn (RQ1 and 2) and how that can be improved with edge self-supervision (RQ3 and 4). We describe each research question and the corresponding experiment design below.

\paragraph{RQ1. Does graph attention learn label-agreement?}

First, we evaluate what the graph attentions of \GATGOb and \GATDPb learn without edge supervision. For this, we present ground-truth of relational importance and a metric to assess graph attention with ground-truth.
\citet{wang2019improving} showed that node representations in the connected component converge to the same value in deep GATs. If there is an edge between nodes with different labels, then it will be hard to distinguish the two corresponding labels with GAT of sufficiently many layers; that is, ideal attention should give all weights to label-agreed neighbors. In that sense, we choose label-agreement between nodes as ground-truth of importance.

We compare label-agreement and graph attention based on Kullback–Leibler divergence of the normalized attention $\valpha_{k} = \left[\alpha_{kk}, \alpha_{k1}, \dots, \alpha_{kJ} \right]$ with label agreement distribution for the center node $k$ and its neighbors $1$ to $J$. The label agreement distribution, $\vell_{k} = \left[ \ell_{kk}, \ell_{k1}, \dots, \ell_{kJ} \right]$ is defined by,
\begin{align}\textstyle
    \ell_{kj} = \hat{\ell}_{kj} / \sum_{s} \hat{\ell}_{ks} ,\quad
    \hat{\ell}_{kj} = 1 \ (\text{if}\ k\ \text{and}\ j\ \text{have the same label})\ \text{or}\ 0\ (\text{otherwise}).
\end{align}
We employ KL divergence in Eq.~\ref{eq:kld}, whose value becomes small when attention captures well the label-agreement between a node and its neighbors.
\begin{equation}\label{eq:kld}
    \text{KLD}(\valpha_{k}, \vell_{k}) = \textstyle
    \sum_{j \in \sN_{k} \cup \{ k \}}
    \alpha_{kj} \log (\alpha_{kj} / \ell_{kj})
\end{equation}

\paragraph{RQ2. Is graph attention predictive of edge presence?}

To evaluate how well edge information is encoded in SuperGAT, we conduct link prediction experiments with \SuperGATGOb and \SuperGATDPb using $\phi_{ij}$ of the last layer as a predictor. We measure the performance by AUC over multiple runs. Since link prediction performance depends on the mixing coefficient $\lambda_{E}$ in Eq.~\ref{eq:full_loss}, we adopt multiple $\lambda_{E} \in \{ 10^{-3}, 10^{-2}, \dots, 10^{3} \}$. We train with an incomplete set of edges, and test with the missing edges and the same number of negative samples. At the same time, node classification performance is measured with the same settings to see how learning edge presence affects node classification.

\paragraph{RQ3. Which graph attention should we use for given graphs?}

The above two research questions explore what different graph attention learns with or without supervision of edge presence. Then, which graph attention is effective among them for given graphs?
We hypothesize that different graph attention will have different abilities to model graphs under various homophily and average degree. We choose these two properties among various graph statistics because they determine the quality and quantity of labels in our self-supervised task. From the perspective of supervised learning of graph attention with edge labels, the learning result depends on \textit{how noisy labels are} (i.e., how low the homophily is) and \textit{how many labels exist} (i.e., how high the average degree is).
So, we generate 144 synthetic graphs (Section~\ref{sec:synthetic-data}) controlling 9 homophily (0.1 -- 0.9) and 16 average degree (1 -- 100) and perform the node classification task in the transductive setting with GCN, \GATGO, \SuperGATSD, and \SuperGATMX.

In RQ3, there are also practical reasons to use the average degree and homophily, out of many graph properties (e.g., diameter, degree sequence, degree distribution, average clustering coefficient). First, the graph property can be computed efficiently even for large graphs. Second, there should be an algorithm that can generate graphs by controlling the property of interest only. Third, the property should be a scalar value because if the synthetic graph space is too wide, it would be impossible to conduct an experiment with sufficient coverage. Average degree and homophily satisfy the above conditions and are suitable for our experiment, unlike some of the other graph properties.


\paragraph{RQ4. Does design choice based on RQ3 generalize to real-world datasets?}

Experiments on synthetic datasets provide an understanding of graph attention models' performance, but they are oversimplified versions of real-world graphs. Can design choice from synthetic datasets be generalized to real-world datasets, considering more complex structures and rich features in real-world graphs? To answer this question, we conduct experiments on 17 real-world datasets with the various average degree (1.8 -- 35.8) and homophily (0.16 -- 0.91), and compare them with synthetic graph experiments in RQ3.


\subsection{Datasets}

\paragraph{Real-world datasets}

We use a total of 17 real-world datasets (Cora, CiteSeer, PubMed, Cora-ML, Cora-Full, DBLP, ogbn-arxiv, CS, Physics, Photo, Computers, Wiki-CS, Four-Univ, Chameleon, Crocodile, Flickr, and PPI) in diverse domains (citation, co-authorship, co-purchase, web page, and biology) and scales (2k - 169k nodes). We try to use their original settings as much as possible. To verify research questions 1 and 2, we choose four classic benchmarks: Cora, CiteSeer, PubMed in the transductive setting, and PPI in the inductive setting. See appendix~\ref{sec:apdx_dataset} for detailed description, splits, statistics (including degree and homophily), and references.


\paragraph{Synthetic datasets}\label{sec:synthetic-data}

We generate random partition graphs of $n$ nodes per class and $c$ classes~\citep{fortunato2010community}, using \texttt{NetworkX} library~\citep{hagberg2008exploring}. A random partition graph is a graph of communities controlled by two probabilities $p_{in}$ and $p_{out}$. If the nodes have the same class labels, they are connected with $p_{in}$, and otherwise, they are connected with $p_{out}$. To generate a graph with an average degree of $d_{avg} = n \cdot \delta$, we choose $p_{in}$ and $p_{out}$ by $p_{in} + (c - 1) \cdot p_{out} = \delta$. The input features of nodes are sampled from overlapping multi-Gaussian distributions~\citep{abu2019mixhop}. We set $n$ to 500, $c$ to 10, and choose $d_{avg}$ between $1$ and $100$, $p_{in}$ from $\{ 0.1\delta, 0.2\delta, \dots, 0.9\delta \}$. We use 20 samples per class for training, 500 for validation and 1000 for test.

\subsection{Experimental Set-up}

We follow the experimental set-up of GAT with minor adjustments. All parameters are initialized by Glorot initialization~\citep{glorot2010understanding} and optimized by Adam~\citep{kingma2014adam}. We apply L2 regularization, dropout~\citep{srivastava2014dropout} to features and attention coefficients, and early stopping on validation loss and accuracy. We use ELU~\citep{clevert2016fast} as a non-linear activation $\rho$. Unless specified, we employ a two-layer SuperGAT with $F = 8$ features and $K = 8$ attention heads (total 64 features). All models are implemented in PyTorch~\citep{paszke2019pytorch} and PyTorch Geometric~\citep{Fey2019Fast}. See appendix \ref{sec:apdx_model} for detailed model and hyperparameter configurations.


\paragraph{Baselines}

For all datasets, we compare our model against representative graph neural models: graph convolutional network (GCN)~\citep{kipf2017semi}, GraphSAGE~\citep{hamilton2017inductive}, and graph attention network (GAT)~\citep{velickovic2018graph}. Furthermore, for Cora, CiteSeer, and PubMed, we choose recent graph neural architectures that learn aggregation coefficients (or discrete structures) over edges: constrained graph attention network (CGAT\footnote{Since CGAT uses node labels in the loss function, it is difficult to use it in semi-supervised learning. So, we modify its auxiliary loss for SSL. See appendix~\ref{sec:apdx_cgat} for details.})~\citep{wang2019improving}, graph learning-convolutional network (GLCN)~\citep{jiang2019semi}, learning discrete structure (LDS)~\citep{franceschi2019learning}, graph agreement model (GAM)~\citep{stretcu2019graph}, and NeuralSparse (NS in short)~\citep{zheng2020robust}. For the PPI, we use CGAT as an additional baseline.


==> ICLR2021 (SuperGAT) (Arxiv)/files/floating_figure.tex <==

\begin{figure*}[t]
  \centering
  \includegraphics[width=9.45cm]{figures/fig_scatter_best_rpg_meta_Avg_Degree_Log10__Homophily_Model_Abs_Gain_percentp_.pdf}
  \vspace{-0.15cm}
  \caption{The best-performed graph attention design for synthetic and real-world graphs with various average degree and homophily.}
  \label{fig:rq3-recipe}
  \vspace{-0.2cm}
\end{figure*}


==> ICLR2021 (SuperGAT) (Arxiv)/files/introduction.tex <==
Graphs are widely used in various domains, such as social networks, biology, and chemistry. Since their patterns are complex and irregular, learning to represent graphs is challenging~\citep{bruna2013spectral, henaff2015deep, defferrard2016convolutional, duvenaud2015convolutional, atwood2016diffusion}.
Recently, graph neural networks (GNNs) have shown a significant performance improvement by generating features of the center node by aggregating those of its neighbors~\citep{zhou2018graph, wu2020comprehensive}.
However, real-world graphs are often noisy with connections between unrelated nodes, and this causes GNNs to learn suboptimal representations.
Graph attention networks (GATs)~\citep{velickovic2018graph} adopt self-attention to alleviate this issue. Similar to attention in sequential data~\citep{luong2015effective, bahdanau2015neural, vaswani2017attention}, graph attention captures the \textit{relational importance of a graph}, in other words, the degree of importance of each of the neighbors to represent the center node.
GATs have shown performance improvements in node classification, but they are inconsistent in the degree of improvement across datasets, and there is little understanding of what graph attention actually learns.

Hence, there is still room for graph attention to improve, and we start by assessing and learning the relational importance for each graph via self-supervised attention. 
We leverage edges that explicitly encode information about the importance of relations provided by a graph. If node $i$ and $j$ are linked, they are more relevant to each other than others, and if node $i$ and $j$ are not linked, they are not important to each other. Although conventional attention is trained without direct supervision, if we have prior knowledge about what to attend, we can supervise attention using them~\citep{knyazev2019understanding,yu2017supervising}. Specifically, we exploit a self-supervised task, using the attention value as input to predict the likelihood that an edge exists between nodes.

To encode edges in graph attention, we first analyze what graph attention learns and how it relates to the presence of edges. In this analysis, we focus on two commonly used attention mechanisms, GAT's original single-layer neural network (GO) and dot-product (DP), as building blocks of our proposed model, self-supervised graph attention network (SuperGAT). We observe that DP attention shows better performance than GO attention in the task to predict link with attention value. On the other hand, GO attention outperforms DP attention in capturing label-agreement between a target node and its neighbors. Based on our analysis, we propose two variants of SuperGAT, scaled dot-product (SD) and mixed GO and DP (MX), to emphasize the strength of GO and DP.

Then, which graph attention models the relational importance best and produces the best node representations? We find that it depends on the average degree and homophily of the graph. We generate synthetic graph datasets with various degrees and homophily, and analyze how the choice of attention affects node classification performance. Based on this result, we propose a recipe to design graph attention with edge self-supervision that works most effectively for given graph characteristics. We conduct experiments on a total of 17 real-world datasets and demonstrate that our recipe can be generalized across them. In addition, we show that models developed by our method improve performance over baselines.

We present the following contributions. First, we present models with self-supervised attention using edge information.
Second, we analyze the classic attention forms GO and DP using label-agreement and link prediction tasks, and this analysis reveals that GO is better at label agreement and DP at link prediction.
Third, we propose recipes to design graph attention concerning homophily and average degree and confirm its validity through experiments on real-world datasets. We make our code available for future research (\url{https://github.com/dongkwan-kim/SuperGAT}).


==> ICLR2021 (SuperGAT) (Arxiv)/files/minipage_table.tex <==

    \begin{table}[t]
        \begin{minipage}[t]{0.6\textwidth}

\centering
\caption{Summary of classification accuracies with 100 random seeds for Cora, CiteSeer, and PubMed. We mark with daggers ($\dagger$) the reprinted results from the respective papers.}
\vspace{-0.2cm}
\label{tab:rq3-transductive}
{\small
\begin{tabular}{llll}
\hline
Model               & Cora                          & CiteSeer         & PubMed                \\ \hline
GCN$^\dagger$       & 81.5                          & 70.3             & 79.0                  \\
GraphSAGE           & 82.1 $\pm$ 0.6                & 71.9 $\pm$ 0.9   & 78.0 $\pm$ 0.7        \\
CGAT                & 81.4 $\pm$ 1.1                & 70.1 $\pm$ 0.9   & 78.1 $\pm$ 1.0        \\
GLCN$^\dagger$      & 85.5                          & 72.0             & 78.3                  \\
LDS$^\dagger$       & 84.1                          & 75               & -                     \\
GCN + GAM$^\dagger$ & 86.2                          & 73.5             & 86.0                  \\ 
GCN + NS$^\dagger$ & 83.7 $\pm$ 1.4         & 74.1 $\pm$ 1.4           & -                    \\ \hline \hline
GAT$^\dagger$    & 83.0 $\pm$ 0.7                & \cellwg72.5 $\pm$ 0.7   & 79.0 $\pm$ 0.4        \\ \hline
\SuperGATSD         & $82.7_{\pm 0.6}^{\downarrow}$ & \cellwg$72.5_{\pm 0.8}$ & $81.3_{\pm 0.5}^{**}$ \\
\SuperGATMX         & \cellwr$\mathbf{84.3}_{\pm 0.6}^{**}$ & \cellwg$\mathbf{72.6}_{\pm 0.8}$ & \cellwr$\mathbf{81.7}_{\pm 0.5}^{**}$ \\ \hline
\end{tabular}
}

        \end{minipage}
        \hfillx
        \begin{minipage}[t]{0.35\textwidth}


\centering
\caption{Summary of micro f1-scores with 30 random seeds for PPI.}
\vspace{-0.2cm}
\label{tab:rq3-inductive}
{\small
\begin{tabular}{ll}
\hline
Model       & PPI                           \\ \hline
GCN         & 61.5 $\pm$ 0.4                \\
GraphSAGE   & 59.0 $\pm$ 1.2                \\
CGAT        & 68.3 $\pm$ 1.7                \\ \hline \hline
GAT      & 72.2 $\pm$ 0.6                \\ \hline
\SuperGATSD & \cellwb$\mathbf{74.4}_{\pm 0.4}^{**}$         \\
\SuperGATMX & $67.2_{\pm 1.2}^{\downarrow}$ \\ \hline
\end{tabular}
}

\vspace{0.22cm}
\fbox{
{\scriptsize
\begin{tabular}{ll}
**            & \pvalue\ $<$ .0001            \\
*             & \pvalue\ $<$ .0005             \\ 
$\downarrow$  & Worse than \GATGO               \\
Color         & Best graph attention (See Fig.~\ref{fig:rq3-recipe})  \\
\end{tabular}
}}

        \end{minipage}
    \vspace{-0.2cm}
    \end{table}

==> ICLR2021 (SuperGAT) (Arxiv)/files/model.tex <==

In this section, we review the original GAT~\citep{velickovic2018graph} and then describe our self-supervised GAT (SuperGAT) models.

\paragraph{Notation}

For a graph $\gG = (V, E)$, $N$ is the number of nodes and $F^{l}$ is the number of features at layer $l$. Graph attention layer takes a set of features $\sH^{l}=\{ \vh_{1}^{l}, \dots, \vh_{N}^{l} \}, \vh_{i}^{l} \in \R^{F^{l}}$ as input and produces output features $\sH^{l+1}=\{ \vh_{1}^{l+1}, \dots, \vh_{N}^{l+1} \}$. 
To compute $\vh_{i}^{l+1}$, the model multiplies the weight matrix $\mW^{l+1} \in \R^{ F^{l+1} \times F^{l} }$ to $\sH^{l}$, linearly combines the features of its first-order neighbors (including itself) $j \in \sN_{i} \cup \{ i \}$ by attention coefficients $\alpha_{ij}^{l+1}$, and finally applies a non-linear activation $\rho$. That is $\vh_{i}^{l+1} = \textstyle \rho \left(\sum_{j \in \sN_{i} \cup \{i\}} \alpha_{i j}^{l+1} \mW^{l+1} \vh_{j}^{l} \right)$. 
We can compute $\alpha_{i j}^{l+1} = \operatorname{softmax}_{j}( \text{LReLU} ( e_{ij}^{l+1} ))$ by normalizing $e_{ij}^{l+1} = a_{e} (\mW^{l+1} \vh_{i}^{l}, \mW^{l+1} \vh_{j}^{l})$ with softmax on $\sN_{i} \cup \{ i \}$ under leaky ReLU activation~\citep{maas2013rectifier}, where $a_{e}$ is a function of the form  $\R^{F^{l+1}} \times \R^{F^{l+1}} \rightarrow \R$.


\paragraph{Graph Attention Forms}

Among two widely used attention mechanisms, the original GAT (GO) computes the coefficients by single-layer feed-forward network parameterized by $\va^{l+1} \in \R^{2F^{l+1}}$. The other is the dot-product (DP) attention,~\citep{luong2015effective, vaswani2017attention} motivated by prior work on node representation learning, and it adopts the same mathematical expression for link prediction score~\citep{tang2015line, kipf2016variational}, 
\begin{align}
    e_{ij, \GO}^{l+1} =  (\va^{l+1})^{\top}\left[\mW^{l+1} \vh_{i}^{l} \| \mW^{l+1} \vh_{j}^{l} \right]
    \quad \text{and}\quad 
    e_{ij, \DP}^{l+1} = 
        (\mW^{l+1} \vh_{i}^{l})^{\top} \bigcdot
        \mW^{l+1} \vh_{j}^{l}.
\end{align}
From now on, we call GAT that uses GO and DP as \GATGOb and \GATDP, respectively.

\input{files/model_figure}

\paragraph{Self-supervised Graph Attention Network}

We propose SuperGAT with the idea of guiding attention with the presence or absence of an edge between a node pair. We exploit the link prediction task to self-supervise attention with labels from edges: for a pair $i$ and $j$, 1 if an edge exists and 0 otherwise. We introduce $a_{\phi}$ with sigmoid $\sigmoid$ to infer the probability $\phi_{ij}$ of an edge between $i$ and $j$.
\begin{align}
    a_{\phi}: \R^{F} \times \R^{F} \rightarrow \R
    \quad \text{and}\quad 
    \phi_{ij} = P \left( (j, i) \in E \right) 
    = \sigmoid (
        a_{\phi} (\mW \vh_{i}, \mW \vh_{j})
    )
\end{align}
We employ four types (GO, DP, SD, and MX) of SuperGAT based on GO and DP attention. For $a_{\phi}$, the form of which is the same as $a_{e}$ in \GATGOb and \GATDP, we name them \SuperGATGOb and \SuperGATDPb respectively. For more advanced versions, we describe \SuperGATSDb (Scaled Dot-product) and \SuperGATMXb (Mixed GO and DP) by unnormalized attention $e_{ij}$ and probability $\phi_{ij}$ that an edge exist between $i$ and $j$.
\begin{align}
\text{\SuperGATSD: }&
e_{ij, \text{SD}} =  e_{ij, \text{DP}} / \sqrt{F},
\quad
\phi_{ij, \text{SD}} = \sigmoid(e_{ij, \text{SD}}). \\
\text{\SuperGATMX: }&
e_{ij, \text{MX}} =  e_{ij, \text{GO}} \cdot \sigmoid(e_{ij, \text{DP}}) ,
\quad
\phi_{ij, \text{MX}} = \sigmoid(e_{ij, \text{DP}}).
\end{align}
\SuperGATSDb divides the dot-product of nodes by a square root of dimension as Transformer~\citep{vaswani2017attention}. This prevents some large values to dominate the entire attention after softmax. \SuperGATMXb multiplies GO and DP attention with sigmoid. The motivation of this form comes from the gating mechanism of Gated Recurrent Units~\citep{learning2014cho}. Since DP attention with the sigmoid represents the probability of an edge, it can softly drop neighbors that are not likely linked while implicitly assigning importance to the remaining nodes.

Training samples are a set of edges $E$ and the complementary set $E^{c} = (V \times V) \setminus{E}$. However, if the number of nodes is large, it is not efficient to use all possible negative cases in $E^{c}$. So, we use negative sampling as in training word or graph embeddings~\citep{mikolov2013efficient, tang2015line, grover2016node2vec}, arbitrarily choosing a total of $p_{n} \cdot |E|$ negative samples $E^{-}$ from $E^{c}$ where the negative sampling ratio $p_{n} \in \R^{+}$ is a hyperparameter.
SuperGAT is capable of modeling graphs that are sparse with a sufficiently large number of negative samples (i.e., $|V \times V| \gg |E|$), but this is generally not a problem because most real-world graphs are sparse~\citep{chung2010graph}.

We define the optimization objective of layer $l$ as a binary cross-entropy loss $\mathcal{L}_{E}^{l}$,
\begin{alignat}{1}
\begin{aligned}
    \mathcal{L}_{E}^{l} = \textstyle
    - \frac{1}{|E \cup E^{-}|}
    \sum_{(j, i) \in E \cup E^{-} }
    \1_{(j, i) = 1} \cdot \log \phi_{ij}^{l}
    + \1_{(j, i) = 0} \cdot \log \left( 1 - \phi_{ij}^{l} \right),
\end{aligned}
\end{alignat}
where $\1_{\cdot}$ is an indicator function. We use a subset of $E \cup E^{-}$ sampled by probability $p_{e} \in (0, 1]$ (also a hyperparameter) at each training iteration for a regularization effect from randomness.

Finally, we combine cross-entropy loss on node labels ($\mathcal{L}_{V}$), self-supervised graph attention losses for all $L$ layers ($\mathcal{L}_{E}^{l}$), and L2 regularization loss, with mixing coefficients $\lambda_{E}$ and $\lambda_{2}$.
\begin{align}\label{eq:full_loss}
    \mathcal{L} \textstyle = \mathcal{L}_{V} + \lambda_{E} \cdot \sum_{l=1}^{L} \mathcal{L}_{E}^{l} + \lambda_{2} \cdot \| \mW \|_{2}.
\end{align}
We use the same form of multi-head attention in GAT and take the mean of each head's attention value before the sigmoid to compute $\phi_{ij}$. Note that SuperGAT has equivalent time and space complexity as GAT. To compute $\mathcal{L}_{E}^{l}$ for one head, we need additional operations in terms of $O(F^{l} \cdot |E \cup E^{-}|)$, and we do not need extra parameters. 


==> ICLR2021 (SuperGAT) (Arxiv)/files/model_figure.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[height=4.4cm]{figures/SuperGAT_model_figures_1.pdf}
  \includegraphics[height=4.4cm]{figures/SuperGAT_model_figures_2.pdf}
  % \vspace{-0.15cm}
  \caption{Overview of attention mechanism of SuperGATs: GO, DP, MX, and SD. Blue circles ($e_{ij}$) represent the unnormalized attention before softmax and red diamonds ($\phi_{ij}$) indicate the probability of edge between node $i$ and $j$. The attention mechanism of the original GAT~\citep{velickovic2018graph} is in the dashed rectangle.}
  \label{fig:model-figure}
  % \vspace{-0.25cm}
\end{figure*}

==> ICLR2021 (SuperGAT) (Arxiv)/files/related_work.tex <==
Deep neural networks are actively studied in modeling graphs, for example the graph convolutional networks~\citep{kipf2017semi} which approximate spectral graph convolution~\citep{bruna2013spectral, defferrard2016convolutional}.
A representative work in a non-spectral way is the graph attention networks (GATs)~\citep{velickovic2018graph} which model relations in graphs using self-attention mechanism~\citep{vaswani2017attention}.
Similar to attention in sequence data~\citep{bahdanau2015neural, luong2015effective, vaswani2017attention}, variants of attention in graph neural networks~\citep{thekumparampil2018attention, Zhang2018GaANGA, wang2019improving, gao2019graphrepresentation, zhang2019adaptive, hou2019measuring} are trained without direct supervision. Our work is motivated by studies that improve attention's expressive power by giving direct supervision~\citep{knyazev2019understanding, yu2017supervising}. Specifically, we employ a self-supervised task to predict edge presence from attention value. This is in line with two branches of recent GNN research: self-supervision and graph structure learning.

Recent studies about self-supervised learning for GNNs propose tasks leveraging the inherent information in the graph structure: clustering, partitioning, context prediction after node masking, and completion after attribute masking~\citep{hu2019strategies, hui2020collaborative, sun2020multi, you2020does}. To the best of our knowledge, ours is the first study to analyze  self-supervised learning of graph attention with edge information. Our self-supervised task is similar to link prediction~\citep{liben2007link}, which is a well-studied problem and recently tackled by neural networks~\citep{zhang2017weisfeiler, zhang2018link}. Our DP attention to predict links is motivated by graph autoencoder (GAE)~\citep{kipf2016variational} and its extensions~\citep{pan2018adversarially, park2019symmetric} reconstructing edges by applying a dot-product decoder to node representations.

Graph structure learning is an approach to learn the underlying graph structure while jointly learning downstream tasks~\citep{jiang2019semi, franceschi2019learning, klicpera2019diffusion, stretcu2019graph, zheng2020robust}. Since real-world graphs often have noisy edges, encoding structure information contributes to learn better representation. However, recent models with graph structure learning suffer from high memory and computational complexity. Some studies target all spaces where edges can exist, so they require $O(|V|^2)$ space and computational complexity~\citep{jiang2019semi, franceschi2019learning}. Others using iterative training (or co-training) between the GNNs and the structure learning model are time-intensive in training~\citep{franceschi2019learning, stretcu2019graph}.
We moderate this problem using graph attention, which consists of parallelizable operations, and our model is built on it without additional parameters. Our model learns attention values that are predictive of edges, and this can be seen as a new paradigm of learning the graph structure.


==> ICLR2021 (SuperGAT) (Arxiv)/files/results.tex <==


This section describes the experimental results which answer the research questions in Section~\ref{sec:experiments}. 
We include a qualitative analysis of attention, quantitative comparisons on node classification and link prediction, and recipes of graph attention design.
The results for sensitivity analysis of important hyper-parameters are in the appendix~\ref{sec:apdx_sensitivity}.


\paragraph{Does graph attention learn label-agreement?}

\textit{GO learns label-agreement better than DP.}

\begin{figure*}[t]
  \centering
  \includegraphics[height=2.55cm]{figures/fig_dist_GAT-Cora-NEDPO8-ES-ATT-NEO8-ES-ATT_KLD_ATT_AGR_-01.pdf}
  \includegraphics[height=2.55cm]{figures/fig_dist_LargeGAT-Cora-NEDPO8-L4-ES-ATT-NEO8-L4-ES-ATT_KLD_ATT_AGR_-01.pdf}
  \vspace{-0.1cm}
  \caption{Distribution of KL divergence between normalized attention and label-agreement on all nodes and layers for Cora dataset (Left: two-layer GAT, Right: four-layer GAT).}
  \label{fig:rq2-result}
  \vspace{-0.2cm}
\end{figure*}


We draw box plots of KL divergence between attention and label agreement distributions of two-layer and four-layer GAT with GO and DP attention for Cora dataset in Figure~\ref{fig:rq2-result}. We see similar patterns in other datasets and place their plots in the appendix~\ref{sec:apdx_label_agreement}. At the rightmost of each sub-figure, we draw the KLD distribution when uniform attention is given to all neighborhoods. Note that the maximum value of KLD of each node is different since the degree of nodes is different. Also, the KLD distribution shows a long-tail shape like a degree distribution of real-world graphs.

There are three observations regarding distributions of KLD. First, we observe that the KLD distribution of GO attention shows a pattern similar to the uniform attention for all citation datasets. This implies that trained GO attention is similar to the uniform distribution, which is in line with previously reported results in the case of entropy\footnote{\url{https://docs.dgl.ai/en/latest/tutorials/models/1_gnn/9_gat.html}}~\citep{wang2019dgl}. Second, KLD values of DP attention tend to be larger than those of GO attention for the last layer, resulting in bigger long-tails. This mismatch between the learned distribution of DP attention and the label agreement distribution suggests that DP attention does not learn label-agreement in the neighborhood. Third, the deeper the model (more than two), the larger the KLD value of DP attention in the last layer. This is because the variance of DP attention increases as the layer gets deeper, as explained below in Proposition~\ref{prop:dp}.


\begin{proposition}\label{prop:dp}
For $l+1$th GAT layer, if $\mathbf{W}$ and $\va$ are independent and identically drawn from zero-mean uniform distribution with variance $\sigma_{w}^{2}$ and $\sigma_{a}^{2}$ respectively, assuming that parameters are independent to input features $\vh^{l}$ and elements of $\vh^{l}$ are independent to each other,
\begin{align}
\scale[0.9]{
\text{Var}[ e_{ij, \text{GO}}^{l+1} ] =  2F^{l+1} \sigma_{w}^{2} \sigma_{a}^{2} \mathbb{E} (\|\vh^{l}\|_{2}^{2})
\ \ \text{and}\ \ 
\text{Var}[ e_{ij, \text{DP}}^{l+1} ] \geq F^{l+1} \sigma_{w}^{4} \left(
    \frac{4}{5} \mathbb{E} \left(
        ((\vh_{i}^{l})^{\top} \vh_{j}^{l})^{2}
    \right)
    + \text{Var} ( (\vh_{i}^{l})^{\top} \vh_{j}^{l} )
\right)
}
\end{align}
\vspace{-0.4cm}
\end{proposition}
The proof is given in the appendix~\ref{sec:apdx_proof}. While the variance of GO depends on the norm of features only, the variance of DP depends on the expectation of the square of input's dot-product and variance of input's dot-product. Stacking GAT layers, the more features of $i$ and $j$ correlate with each other, the larger the input's dot-product will be. After DP attention is normalized by softmax, which intensifies the larger values among them, normalized DP attention attends to only a small portion of the neighbors and learns a biased representation.


\paragraph{Is graph attention predictive for edge presence?}

\textit{DP predicts edge presence better than GO.}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.93\textwidth]{figures/fig_line_perf_against_att_lambda_real_world_datasets_GAT_and_Task_GAT_and_Task_Dataset.pdf}
  \vspace{-0.2cm}
  \caption{Test performance on node classification and link prediction for GO and DP attentions against the mixing coefficient $\lambda_{E}$. We report accuracy (Cora, CiteSeer, PubMed) and micro f1-score (PPI) for node classification, and AUC for link prediction.}
  \label{fig:rq1-result}
  \vspace{-0.25cm}
\end{figure*}

In Figure~\ref{fig:rq1-result}, we report the mean AUC over multiple runs (5 for PPI and 10 for others) for link prediction (red lines) and node classification (gray lines).
As the mixing coefficient $\lambda_{E}$ increases, the link prediction score increases in all datasets and attentions. This is a natural result considering that $\lambda_{E}$ is the weight factor of self-supervised graph attention loss ($\mathcal{L}_{E}$ in Equation~\ref{eq:full_loss}).
For three out of four datasets, DP attention outperforms GO for link prediction for all range of $\lambda_{E}$ in our experiment.
Surprisingly, even for small $\lambda_{E}$, DP attention shows around 80 AUC, much higher than the performance of GO attention.
PPI is an exception where GO attention shows higher performance for small $\lambda_{E}$ than DP, but the difference is slight.
The results of this experiment demonstrate that DP attention is more suitable than GO attention in encoding edges.

This figure also includes node classification performance. 
For all datasets except PubMed, we observe a trade-off between node classification and link prediction; that is, node classification performance decreases in \SuperGATGOb and \SuperGATDPb as $\lambda_{E}$ increases and thus link prediction performance increases. 
PubMed also shows a decrease in performance at the largest $\lambda_{E}$ we have tested. 
This implies that it is hard to learn the relational importance from edges by simply optimizing graph attention for link prediction.

\paragraph{Which graph attention should we use for given graphs?}

\textit{It depends on homophily and average degree of the graph.}

\begin{figure*}[t]
  \centering
  \includegraphics[height=3.1cm]{figures/fig_line_analysis_rpg_part135_Model_Model_Homophily.pdf}
  \includegraphics[height=3.1cm]{figures/fig_line_analysis_rpg_part79_Model_Model_Homophily.pdf}
  \vspace{-0.2cm}
  \caption{Mean test accuracy gains (of 5 runs) against \GATGOb on synthetic datasets, varying homophily and average degree of the input graph.}
  \label{fig:rq3-synthetic-result}
  \vspace{-0.45cm}
\end{figure*}

In Figure~\ref{fig:rq3-synthetic-result}, we draw the mean test accuracy gains (over 5 runs) against \GATGOb as the average degree increases from 1 to 100, for different values of homophily, on 64 synthetic graphs with GCN, \SuperGATSD, \SuperGATMX. See full results from appendix~\ref{sec:apdx_synthetic}. We define homophily $h$ as the average ratio of neighbors with the same label as the center node~\citep{pei2019geom}. That is $h = \textstyle \frac{1}{|V|} \sum_{i \in V} \left( \sum_{j \in \sN_{i}} \1_{l(i) = l(j)} \big/  |\sN_{i}| \right)$, where $l(i)$ is the label of node $i$. The expectation of homophily for random partition graphs is analytically $p_{in} / \delta$, and we just adopt this value to label the homophily of graphs in Figure~\ref{fig:rq3-synthetic-result}.

We make the following observations from this figure. First, if the homophily is low ($\leq 0.2$), \SuperGATSDb performs best among models because DP attention tends to focus on a small number of neighbors. This result empirically confirms what we analytically found in Proposition~\ref{prop:dp}. Second, even when homophily is low, the performance gain of SuperGAT against GAT increases as the average degree increases to a certain level (around 10), meaning relation modeling can benefit from self-supervision if there are sufficiently many edges providing supervision. This is in agreement with prior study of label noise for deep neural networks where they find that the absolute amount of data with correct labels affects the learning quality more than the ratio between data with noisy and correct labels~\citep{rolnick2017deep}. Third, if the average degree and homophily are high enough, there is no difference between all models, including GCNs. If there are more correct edges beyond a certain amount, we can learn fine representation without self-supervision. Most importantly, if the average degree is not too low or high and homophily is above $0.2$, \SuperGATMXb performs better than or similar to \SuperGATSD. This implies that we can take advantage of both GO attention to learn label-agreement and DP attention to learn edge presence by mixing GO and DP. Note that many of the real-world graphs belong to this range of graph characteristics.

The results on synthetic graphs imply that understanding of graph domains should be preceded to design graph attention. That is, by knowing the average degree and homophily of the graphs, we can choose the optimal graph attention in our design space.

\paragraph{Does design choice based on RQ3 generalize to real-world datasets?}

\textit{It does for 15 of 17 real-world datasets.}




\input{files/big_table}
\input{files/minipage_table}

\input{files/floating_figure}



In Figure~\ref{fig:rq3-recipe}, we plot the best-performed graph attention for synthetic graphs with square points in the plane of average degree and homophily. The size is the performance gain of SuperGAT against GAT, and the color indicates the best model. If the difference is not statistically significant (\pvalue\ $\ge$ .05) between GAT and SuperGAT, and between \SuperGATMXb and \SuperGATSD, we mark as GAT-Any and SuperGAT-Any, respectively. We call this plot a recipe since it introduces the optimal attention to a specific region's graph.

Now we map the results of 17 real-world datasets in Figure~\ref{fig:rq3-recipe} according to their average degree and homophily. Average degree and homophily can be found in the appendix~\ref{sec:apdx_dataset}, and experimental results of graph attention models are summarized in Tables~\ref{tab:real-world-many}, \ref{tab:rq3-transductive} and \ref{tab:rq3-inductive}. We report the mean and standard deviation of performance over multiple seeds (30 for graphs with more than 50k nodes and 100 for others). We put unpaired t-test results of SuperGAT with \GATGOb with asterisks.

We find that the graph attention recipe based on synthetic experiments can generalize across real-world graphs. PPI and Four-Univ (\textcolor{strongblue}{$\blacktriangle$}) are surrounded by squares of \SuperGATSDb (\textcolor{middleblue}{$\blacksquare$}) at the bottom of the plane. Wiki-CS (\textcolor{strongpurple}{$\blacktriangle$}), located in the SuperGAT-Any region (\textcolor{middlepurple}{$\blacksquare$}), also show no difference in performance between SuperGATs. Nine datasets (\textcolor{strongred}{$\blacktriangle$}), which \SuperGATMXb shows the highest performance, are located in the MX regions (\textcolor{middlered}{$\blacksquare$}) or within the margin of two squares. Note that there are two MX regions: lower-middle average degree (2.5 - 7.5) and high homophily (0.8 - 0.9), and upper-middle average degree (7.5 - 50) and lower-middle homophily (0.3 - 0.5). There are five datasets with no significant performance change across graph attention ($\blacktriangle$). CiteSeer, Photo, and Computers are within a margin of one square from the GAT-Any region (\textcolor{middlegray}{$\blacksquare$}); however, Flickr and Crocodile are in the SuperGAT-Any region. To find out the cause of this irregularity, we examine the distribution of degree and per-node homophily (appendix~\ref{sec:apdx_dist_degree_and_homophily}). We observe a more complex mixture distribution of homophily and average degree in Flickr and Crocodile, and this seems to be equivalent to mixing graphs of different characteristics, resulting in inconsistent results with our attention design recipe.


\paragraph{Comparison with baselines}

For a total of 17 datasets, SuperGAT outperforms GCN for 13 datasets, GAT for 12 datasets, GraphSAGE for 16 datasets. Interestingly, for CS, Physics, Cora-ML, and Flickr, in which our model performs worse than GCN, GAT also cannot surpass GCN.
It is not yet known when the degree-normalized aggregation of GCN outperforms the attention-based aggregation, and more research is needed to figure out how to embed the degree information into graph attention.
Tables~\ref{tab:rq3-transductive} and \ref{tab:rq3-inductive} show performance comparisons between SuperGAT and recent GNNs for Cora, CiteSeer, PubMed, and PPI. Our model performs better for CiteSeer (0.6\%p) and PubMed (3.4\%p) than GLCN, which gives regularization to all relations in a graph. GCN + NS (NeuralSparse) performs better than our model for CiteSeer (1.5\%p) but not for Cora (0.6\%p). CGAT modified for semi-supervised learning shows lower performance than GAT. Although LDS and GAM which use iterative training show better performance except for LDS on Cora, these models require significantly more computation for the iterative training. For example, GCN + GAM compared to our model needs more $\times 34$ more training time for Cora, $\times 72$ for CiteSeer, and $\times 82$ for PubMed. See appendix~\ref{sec:apdx_wall_clock_time} and \ref{sec:apdx_wall_clock_time_result} for the experimental set-up and the result of wall-clock time analysis.


==> ICLR2021 (SuperGAT) (Arxiv)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\valpha{{\bm{\alpha}}}
\def\vell{{\bm{\ell}}}

\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

